State Space Models for Event Cameras

Today, state-of-the-art deep neural networks that process event-camera data first convert a temporal window of events into dense, grid-like input representations. As such, they exhibit poor generalizability when deployed at higher inference frequencies (i.e., smaller temporal windows) than the ones they were trained on. We address this challenge by introducing state-space models (SSMs) with learnable timescale parameters to event-based vision. This design adapts to varying frequencies without the need to retrain the network at different frequencies. Additionally, we investigate two strategies to counteract aliasing effects when deploying the model at higher frequencies. We comprehensively evaluate our approach against existing methods based on RNN and Transformer architectures across various benchmarks, including Gen1 and 1 Mpx event camera datasets. Our results demonstrate that SSM-based models train 33% faster and also exhibit minimal performance degradation when tested at higher frequencies than the training input. Traditional RNN and Transformer models exhibit performance drops of more than 20 mAP, with SSMs having a drop of 3.76 mAP, highlighting the effectiveness of SSMs in event-based vision tasks.

==> sec/5_limitations.tex <==
\section{Limitations}
\label{sec:limitations}
\vspace{-1ex}
The model's adaptability to varying frequencies, despite being superior to existing methods, is not absolute. Performance drop still occurs at extremely high frequencies, indicating room for further improvement, which is the next step to tackle. Additionally, our model's complexity, especially in integrating SSMs with ViT, might pose challenges in computational resources. It would be interesting to see whether a pure SSM-based model can achieve high performance.

==> sec/subsec/h2norm_bak.tex <==
\subsubsection{$\textbf{H}_{\textbf{2}}$ norm}
\label{sec:method:low_pass_bandlimiting:h2_norm}
Another strategy for solving aliasing problem includes minimizing $H_{2}$ norm of the continuous time matrices A, B and C by including it as term in the loss function.
The $H_{2}$ norm of a system is a fundamental measure of its performance and stability. We describe a computational approach to estimate the $H_{2}$ norm for SSMs with continuous matrices \( \mathbf{A}, \mathbf{B}, \) and \( \mathbf{C} \).

Given a system described by matrices \( \mathbf{A}, \mathbf{B}, \) and \( \mathbf{C} \), the transfer function \( \mathbf{G}(s) \) from the Laplace transform can be defined in the frequency domain as:

\begin{equation}
\mathbf{G}(j\omega) = \mathbf{C} (j\omega \mathbf{I} - \mathbf{A})^{-1} \mathbf{B},
\end{equation}

where \( j\omega \) denotes the imaginary unit times the angular frequency, and \( \mathbf{I} \) is the identity matrix. The $H_{2}$ norm is computed as the integral of the squared magnitude of the frequency response over the range of interest, typically the entire frequency spectrum.

To numerically estimate this integral, we discretize the frequency range \( [\omega_{\text{min}}, \omega_{\text{max}}] \) into \( N \) points and apply numerical integration methods to the squared Frobenius norm of \( \mathbf{G}(j\omega) \). This yields an approximate $H_{2}$ norm of the system:

\begin{equation}
\left\| \mathbf{G} \right\|_{H_2} \approx \sqrt{\frac{1}{\pi} \sum_{k=1}^{N} \left\| \mathbf{G}(j\omega_k) \right\|_F^2 \Delta \omega },
\end{equation}

where \( \Delta \omega \) is the frequency step size and \( \left\| \cdot \right\|_F \) denotes the Frobenius norm. The choice of numerical integration scheme—rectangle, trapezoid, or Simpson's rule—affects the accuracy of the approximation.

%\begin{itemize}
%    \item Rectangle rule approximates the integral by the sum of areas of rectangles under the curve.
%    \item Trapezoid rule uses trapezoids to approximate the area under the curve, improving accuracy.
%    \item Simpson's rule offers a higher-order approximation by fitting parabolas to segments of the curve.
%\end{itemize}

For the Simpson's rule, an odd number of points is required to ensure that each segment can be paired. In our implementation, we leverage the parallel computing capabilities of PyTorch to vectorize the computation across frequency points, significantly reducing computational time. The final normalization step adjusts the scale of the $H_{2}$ norm to account for different system dimensions and ensures comparability across various system sizes.

This computational framework is integral for analyzing the robustness of SSMs, providing insights into the stability and dynamic properties of models.
